String Diagram Rewrite Theory III: Confluence with and without Frobenius

In this paper we address the problem of proving confluence for string diagram rewriting, which was previously shown to be characterised combinatorically as double-pushout rewriting with interfaces (DPOI) on (labelled) hypergraphs. For standard DPO rewriting without interfaces, confluence for terminating rewrite systems is, in general, undecidable. Nevertheless, we show here that confluence for DPOI, and hence string diagram rewriting, is decidable. We apply this result to give effective procedures for deciding local confluence of symmetric monoidal theories with and without Frobenius structure by critical pair analysis. For the latter, we introduce the new notion of path joinability for critical pairs, which enables finitely many joins of a critical pair to be lifted to an arbitrary context in spite of the strong non-local constraints placed on rewriting in a generic symmetric monoidal theory.

==> part3source-revised/Background.tex <==
% -*- root: ../main.tex -*-

%$f\colon a\to b$



\paragraph{Notation.}
%$\catC[a,b]$ is the set of arrows from $a$ to $b$ in a small category $\catC$, composition of $f \colon a \to b$, $g\colon b \to c$ is written $f\poi g \colon a \to c$.
The composition of arrows $f \colon a \to b,\, g\colon b \to c$ in a category $\catC$
is written as $f\poi g$.
% \colon a \to c$.
For $\catC$ symmetric monoidal, $\tns$ is its monoidal product and $\sigma_{a,b} \colon a \tns b \to b \tns a$ is the symmetry for 
objects $a,b \in \catC$. %Given $\funF \colon \catC_1 \to \catC_2$, we denote with $\funF^{\op} \colon \catC_1^{\op}\to \catC_2^{\op}$ the induced functor on the opposite categories of $\catC_1, \catC_2$.
%Given $\catC$ with pushouts, its cospan bicategory has the objects of $\catC$ as $0$-cells, cospans of arrows of $\catC$ as $1$-cells and cospan morphisms as $2$-cells; $\Cospan{\catC}$ is the \emph{category} obtained by identifying iso $1$-cells and forgetting the $2$-cells.


\subsection{DPO rewriting}\label{ssec:DPOrewriting}
\input{part3source-revised/bDPOrewriting.tex}

\subsection{PROP rewriting}\label{ssec:PROPrewriting}
\input{part3source-revised/PROPrewriting.tex}


%\subsection{From PROP to DPO rewriting with interfaces}\label{ssec:PROPDPOrewriting}
%\input{source/PROPDPOrewriting.tex}


==> part3source-revised/convexity.tex <==
%\section{Local confluence and convex rewriting}

For $G$ directed acyclic and monogamous, we call \emph{inputs} the nodes of $G$ that do not have any ingoing edge, and \emph{outputs} those that do not have any outgoing edge. This yields a canonical discrete interface $n+m \to G$ for $G$ with $n$ inputs and $m$ outputs.

\begin{definition} A graph $G$ is \emph{strongly connected} if every input has a forward path to any output. A rewriting rule is \emph{good}\fznote{substitute good with appropriate name} if if it of the form $L \tl{f} i+j \tr{} R$, where $L$ and $R$ are monogamous directed acyclic graphs, $L$ is strongly connected and $f$ is a mono. 
\end{definition}

\begin{lem}\label{lemma:connected->convex} For $L \tl{f} i+j \tr{} R$ good, any matching $m$ in a monogamous directed acyclic graph $G$ as below must be convex.
\[
\xymatrix{
L \ar[d]_{m} & \ar[l]_{f} i+j \ar[r] \ar[d] & R \\
G & \ar[l] C
}
\]
\end{lem}
\begin{proof} For $m$ being convex means that (i) $m$ is an embedding and (ii) the image of $m$ is a convex subgraph.

For (i), observe that the above square being a pushout implies that $m$ is injective on the edges of $L$: indeed, edges of $L$ could only be identified if they were in the image of $f : i+j \to L$, but $i+j$ is discrete. For nodes $n_1$ and $n_2$, we distinguish the following cases.
\begin{itemize}
\item If $n_1 \in s(e_1)$ and $n_2 \in s(e_2)$, for some edges $e_1$ and $e_2$, then $m(e_1) \neq m(e_2)$ implies $m(n_1) \neq m(n_2)$, by monogamicity.
\item If $n_1 \in t(e_1)$ and $n_2 \in t(e_2)$, the same reasoning holds.
\item If $n_1 \in s(e_1)$ and $n_2 \in t(e_2)$, with $n_1$ input and $n_2$ output node, then identifying them would create a cycle in $G$.
\item If $n_1 \in s(e_1)$ and $n_2 \in t(e_2)$, with either $n_1$ not input or $n_2$ not output, then identifying them would violate monogamicity of $G$.
\item In the remaining case, one of the two nodes is neither in the source nor in the target of any edge, thus is both an input and an output. This cannot be the case, because $f$ must be injective and thus $f[i]$ and $f[j]$ are disjoint.
\end{itemize}
For (ii), take any two nodes $m(n_1)$ and $m(n_2)$ in the image of $m$ and consider a forward path $\pi$ from $m(n_1)$ to $m(n_2)$. Suppose for a contradiction that $\pi$ is not in the image of $m$. This mean that some segment $\tau$ of $\pi$ is not in the image of $m$, i.e.
$$m(n_1) \tr{\pi} m(n_2) = m(n_1) \tr{m(\sigma)} m(n_3) \tr{\tau} m(n_4)  \tr{m(\rho)} m(n_2).$$
Because both $G$ and $L$ are monogamous, then there is no outgoing edge in $L$ from $n_3$, and no ingoing edge in $L$ to $n_4$. \fbnote{This is a bit too fast: explain it better} By monogamicity of $L$, this means that $n_3$ is an output node and $n_4$ is an input node of $L$. Therefore by strong connectedness there is a path $\pi'$ from $n_4$ to $n_3$ in $L$. But then the composite $m(\tau) ; \tau$ yields a cycle in $G$, contradiction. \end{proof}

\begin{prop} \label{prop:connected->DPO=convex} Let $n \tr{} G \tl{} m$ be a monogamous directed acyclic cospan. For $L \tl{f} i+j \tr{} R$ good, any DPO rewriting step
\[
\xymatrix@R=15pt@C=20pt{
L \ar[d]_{f}   &  i+j \ar[d]
 \ar@{}[dl]|(.8){\text{\large $\urcorner$}}
 \ar@{}[dr]|(.8){\text{\large $\ulcorner$}}
 \ar[l]_{[a_1,a_2]} \ar[r]^{[b_1,b_2]}  & R \ar[d] \\
 D &  C \ar[l] \ar[r]  & E \\
&  n+m \ar[u] \ar[ur]_{[p_1,p_2]}  \ar[ul]^{[q_1,q_2]}
}
\]
is also a convex rewriting step.
\end{prop}
\begin{proof}[proof sketch]
There are two conditions to check. The first is that the matching $m$ is convex, which is guaranteed by Lemma~\ref{lemma:connected->convex}. The second is that $C$ is the boundary complement, see Definition 5.1 in the LICS paper. For that, the crucial observation is provided by Lemma 3.11 in LICS: given a monogamous $G$ and a convex matching as above, it allows to decompose $G$ in terms of $L$ and its boundary complement $C'$. \fbnote{This step is wrong. You have not proved yet that $C$ is the boundary complement. It is clearly the pushout complement (which is unique because of left injectivity of the rule) but it might not be a boundary complement. Right? I guess that the solution is simple, but should be slightly reformulated. Also the notion of boundary complement involve the whole cospan and not only $C$.} Because pushout complements are unique for left-injective rules, we can conclude that $C = C'$.
\end{proof}


\begin{definition} A critical pair
\[
\vcenter{
    \xymatrix@R=15pt{
    R_1 \ar[d] & \ar[l] K_1 \dlcorner  \ar[d] \ar[r] & L_1 \ar@{}[dr]|(.8){\text{\large $\ulcorner$}\qquad\quad} \ar[dr]^{f_1} && \ar[dl]_{f_2} \ar@{}[dl]|(.8){\qquad\quad\text{\large $\urcorner$}} L_2 & \ar[l] K_2 \ar[d] \drcorner\ar[r] & R_2 \ar[d] \\
    H_1  & \ar[l] C_1 \ar[rr] & & S \ar@{}[d]|(.7){\text{\large $\dcorner$}} & & \ar[ll] C_2  \ar[r] & H_2 \\
    &&& \ar@/^/[ull] J \ar@/_/[urr] & & &
    }
}
\]
is \emph{good} if the two rules are good and $S$ is monogamous directed acyclic.
\end{definition}

\begin{example} Example of with $S$ \emph{not} monogamous:
\[ L_1 = \bullet \tr{f} \bullet \qquad L_2 = \bullet \tr{g} \bullet \qquad S = \xymatrix{ \bullet \ar@/^/[r]^{f} \ar@/_/[r]_{g} & \bullet }
\]
We don't want to consider such critical pairs when doing critical pair analysis for the syntax.
\end{example}

For interpreting the confluence problem for PROP rewriting, this is the relevant theorem.

\begin{theorem} For a rewriting system only consisting of good rules, the following are equivalent:
\begin{itemize}
\item All good critical pairs are joinable.
\item The rewriting system is locally confluent on monogamous directed acyclic cospans. Furthermore, all DPO rewriting steps involved are convex.
\end{itemize}
\end{theorem}
\begin{proof}[proof sketch]
For the non-trivial direction, suppose that all good critical pairs are joinable. The proof follows the same steps as the one of Theorem~\ref{th:locconfl}. The essential bit is to check that, starting with $n \tr{} G_0 \tl{} m$ monogamous directed acyclic (where $n+m = I$), the critical pair to consider at the first step is good. For this to hold, the graph $G_0'$ obtained by epi-mono factorisation from $G_0$ must be monogamous directed acyclic: but this is immediate, because it embeds by construction in $G_0$ with those properties.

All the remaining steps of the proof should pose no problem \fznote{To be checked more carefully}: indeed, the clipping and the embedding construction simply construct more DPO rewriting steps, that by Proposition~\ref{prop:connected->DPO=convex} are also convex.
\end{proof} 

\begin{lem}\label{lemma:keyconvex}
 Let $(G'\tl{f'}J')$ and $(G\tl{f}J)$ be two monogamous directed acyclic graphs with interface. Suppose that $f'$ is mono. If there exists a mono $m\colon G' \to G$ then there exist a $\Sigma$-hypergraph $C$ and morphisms $J'\tr{}C$ and $J\tr{}C\tr{}G$ making the following diagram commute and the square $(\dagger)$ below a pushout.
\begin{equation}\label{diag:embeddingAssumption}
\begin{aligned}
\xymatrix{
& J' \ar[r]^{f'} \ar[d] \ar@{}[dr]|(.5){(\dagger)} & G' \ar[d]^m \\
J  \ar[r]  \ar@/_10pt/[rr]_f 
& C  \ar[r] & G
}
\end{aligned}
\end{equation}
\end{lem}
\begin{proof}
For an arbitrary hypergraph $H$, we denote  by $V_H$ and $E_H$ its sets of nodes and hyperedges, respectively. 

We define $C$ as the $\Sigma$-hypergraph having as set of nodes $V_G \setminus m(V_{G'} \setminus f'(V_{J'}))$ and as set of hyperedges $E_G \setminus m(E_{G'})$. Then, there are evident embeddings of $J'$ into $C$ and $C$ into $G$. For $m$ and $f$ mono, this is the standard calculation of the pushout complement, so to prove that $(\dagger)$ is a pushout we need only show that $C$ is well-defined. This is true whenever $m$ satisfies the gluing conditions, namely no hyperedge in $E_G \setminus  m(E_{G'})$ has a source or target in $V_G \setminus m(V_{G'} \setminus f'(V_{J'}))$. Now, nodes $v$ in $V_{G'} \setminus f'(V_{J'})$ are internal nodes of $G'$, so by monogamy, $m(v)$ must have a unique in- and out-hyperedge, both in the image of $m$. In particular, these hyperedges cannot be in $E_G \setminus  m(E_{G'})$.

To prove the statement we only need to show the existence of $J\tr{g}C$ making the lower part of the above diagram commute. 
We can take $g(v)= f(v)$ for all vertex $v \in J$. This is well defined since $f(v) \notin m(V_{G'} \setminus f' (V_{J'}))$: as discussed above, all nodes $v' \in V_{G'} \setminus f'(V_{J'})$ should be internal in $G$, so by monogamy $m(v')$ should have exactly one in and out hyperdege and it cannot be in the image of the interface $J$.
\end{proof}

\begin{theorem}
If all pre-critical pairs are joinable then rewriting is locally confluent.
\end{theorem}
 \begin{theorem}[Local confluence] \label{th:locconfl} If all the pre-critical pairs are joinable then the rewriting is locally confluent. That means, given $(G_0 \tl{} I)$ rewriting into $(G_{1,1} \tl{} I)$ and $(G_{1,2} \tl{} I)$, there exists $(W \tl{} I)$ such that
 \[
\xymatrix@R=5pt@C=10pt{
&  \ar@{=>}[dl]  (G_0 \tl{} I) \ar@{=>}[dr] & \\
(G_{1,1} \tl{} I) \ar@{=>}[dr]^>>>{*} && (G_{1,2} \tl{} I) \ar@{=>}[dl]_>>>{*} \\
&(W \tl{} I).&
}
\]
 \end{theorem}

\begin{proof}
 By assumption we have the following two rewriting steps from $(G_0\tl{} I)$.
$$\xymatrix@R=15pt{
    R_{1,1} \ar[d] & \ar[l] K_{1,1} \dlcorner  \ar[d] \ar[r] & L_{1,1} \ar@{}[dr]|(.8){\text{\large $\ulcorner$}\qquad\quad} \ar[dr]^{f_1} && \ar[dl]_{f_2} \ar@{}[dl]|(.8){\qquad\quad\text{\large $\urcorner$}} L_{1,2} & \ar[l] K_{1,2} \ar[d] \drcorner\ar[r] & R_{1,2} \ar[d] \\
    G_{1,1}  & \ar[l] C_{1,1} \ar[rr] & & G_0  & & \ar[ll] C_{1,2}  \ar[r] & G_{1,2} \\
    &&& \ar@/^/[ull] I \ar[u] \ar@/_/[urr] & & &
    }$$

By epi-mono factorization of $[f_1,f_2]\colon L_{1,1}+L_{1,2} \to G_0$ we have
  $$ \vcenter{
    \xymatrix@R=15pt@C=5pt{
    L_{1,1} \ar[rd] \ar@(d,ul)[rdd]_{f_1} & & L_{1,2} \ar[ld] \ar@(d,ur)[ldd]^{f_2} \\
    & G_0' \ar@{_{(}->}[d] \\
    & G_0
    }
}$$
%\fgnote{sign mono arrows}


We apply Construction~\ref{constr:clipping} twice:

$$ \scalebox{.8}{    \xymatrix@R=10pt@C=10pt{
  &  R_{1,1} \ar[dd]|\hole \ar[dl] & &  \ar[ll] K_{1,1} \ar[dl]  \ar[dd]|\hole \ar[rr] & &  L_{1,1} \ar[drr] \ar@/_1pc/[ddrr]|(.36)\hole && && \ar@/^1pc/[ddll]|(.36)\hole  L_{1,2} \ar[dll] & &  \ar[ll] K_{1,2}  \ar[dr] \ar[rr] \ar[dd]|\hole && R_{1,2} \ar[dr] \ar[dd]|\hole \\
  H_{1,1}' \ar[dr] && C_{1,1}' \ar[dr] \ar[ll]  \ar[rrrrr] & & & & & G_0' \ar[d] & & &&& C_{1,2}' \ar[dl]  \ar[lllll] \ar[rr] && H_{1,2}'   \ar[dl]\\
  &  H_{1,1}  & & \ar[ll] C_{1,1} \ar[rrrr] && & & G_0 && & & \ar[llll] C_{1,2}  \ar[rr] & & H_{1,2} \\
  & &&& &&& \ar@/^/[ullll] I \ar[u] \ar@/_/[urrrr] & & &
    }
}$$

Now $G_0'$ is a monogamous directed acyclic hypergraph, since it is embedded into $G_0$ which is monogamous directed acyclic.
Therefore there exist some $J_0' \tr{f'} G_0'$ that is a monogamous directed acyclic hypergraph with interface. We can apply twice Lemma \ref{lemma:keyconvex} to 
 $$ \scalebox{.8}{
    \xymatrix@R=10pt@C=10pt{
   K_{1,1}   \ar[rr]^{l_1} & &  L_{1,1} \ar[drr]^{f_1'}  && &&   L_{1,2} \ar[dll]_{f_1'} & &  \ar[ll]_{l_2} K_{1,2} \\
&  & & & G_0'   \\
 & &   & &  J' \ar[u]^{f'}
}}$$
since $l_i$ and $f_i'$ are mono for $i=1,2$. By uniqueness of pushout complement we have that the following diagram commute.
 $$ \scalebox{.8}{
    \xymatrix@R=10pt@C=10pt{
  &  R_{1,1}  \ar[dl] & &  \ar[ll] K_{1,1} \ar[dl]  \ar[rr] & &  L_{1,1} \ar[drr]  && &&   L_{1,2} \ar[dll] & &  \ar[ll] K_{1,2}  \ar[dr] \ar[rr]  && R_{1,2} \ar[dr] \\
  G_{1,1}'  && C_{1,1}'  \ar[ll]  \ar[rrrrr] & & & & & G_0'  & & &&& C_{1,2}'  \ar[lllll] \ar[rr] && G_{1,2}'   \\
  &   & &  && & & J' \ar[u]^f \ar@/^5pt/[ulllll] \ar@/_5pt/[urrrrr] && & &    }
}$$
This is a pre-critical pair. By assumption, it is joinable, that is we have derivations $$(G_{1,1}' \tl{} J') \rewr^* (W' \tl{\beta'} J' ) \tlrewr (G_{1,2}' \tl{} J') \text{.}$$
Suppose now that the leftmost derivation requires $n$ steps and the rightmost $m$. To keep the notation consistent with the embedding construction, we fix notation $G_{n,1}' \df W' {=:} \ G_{m,2}'$.

We would like to use now Construction~\ref{constr:embedding}. In order to do so, we need once more Lemma \ref{lemma:keyconvex}. In the following diagram $m$ is mono by construction.
 $$ \scalebox{.8}{
    \xymatrix@R=10pt@C=10pt{
   J' \ar[r]^{f'}  & G_0' \ar[d]^m \\
J \ar[r]  & G_0   
}}$$
To prove that $f'$ is also mono, observe that by monogamicity of $G_0'$ either it contains an isolated node, or $f'$ is mono. We prove that $G_0'$ cannot contain an isolated node. Indeed, if it contains an isolated node, this should be either in $L_{1,1}$ or in $L_{2,2}$, since $L_{1,1}+L_{2,2}\to G_0'$ is epi by construction. But this is impossible because $K_{i,i} \to L_{i,i}$ is mono by assumption.
Therefore we can use Lemma \ref{lemma:keyconvex} to obtain 
\begin{equation*}
\begin{aligned}
\xymatrix{
& J' \ar[r]^{f'} \ar[d]_{\xi} \ar@{}[dr]|(.5){(\dagger)} & G' \ar[d]^m \\
J  \ar[r]^{\zeta}  \ar@/_10pt/[rr]_f 
& C  \ar[r] & G
}
\end{aligned}
\end{equation*}
and apply Construction~\ref{constr:embedding}, which yields
$$(G_0 \tl{} J) \rewr (G_{1,1} \tl{} J) \rewr^* (G_{n,1} \tl{\beta_1} J )$$
 extending $(G_0' \tl{} J') \rewr (G_{1,1}' \tl{} J') \rewr^* (G_{n,1}' \tl{\beta'} J' )$
   and
  $$(G_0 \tl{} J) \rewr (G_{1,2} \tl{} J) \rewr^* (G_{m,2} \tl{\beta_2} J )$$
   extending $(G_0' \tl{} J') \rewr (G_{1,1}' \tl{} J') \rewr^* (G_{m,2}' \tl{\beta'} J' )$.


 The next step is to prove that $(G_{n,1} \tl{\beta_1} J ) \cong (G_{m,2} \tl{\beta_2} J ) $. To see this, it is enough to observe that both the following  squares are pushouts of 
 \[ C \tl{\xi} J' \tr{\beta'} W'=G_{n,1}'=G_{m,2}'.\]
 $$
 \xymatrix{
 J' \ar[d]_\xi \ar[r]^{\beta'} & G_{n,1}' \ar[d] \\
 C \ar[r]_{\beta_1'} & G_{n,1}
 }
 \qquad
 \xymatrix{
 J' \ar[d]_\xi \ar[r]^{\beta'} & G_{m,2}' \ar[d] \\
 C \ar[r]_{\beta_2'} & G_{m,2}
 }
$$
Indeed, the leftmost is a pushout by composition of squares $(\epsilon_n)$ and $(\delta_n)$ in the embedding construction and the rightmost by composition of $(\epsilon_m)$ and $(\delta_m)$. We conclude by observing that, by Construction~\ref{constr:embedding}, $\beta_i = \zeta ; \beta_i'$ for $i=1,2$. 
\end{proof}


